SEM-Net: Efficient Pixel Modelling for image inpainting with Spatially Enhanced SSM

Image inpainting aims to repair a partially damaged image based on the information from known regions of the images. \revise{Achieving semantically plausible inpainting results is particularly challenging because it requires the reconstructed regions to exhibit similar patterns to the semanticly consistent regions}. This requires a model with a strong capacity to capture long-range dependencies. Existing models struggle in this regard due to the slow growth of receptive field for Convolutional Neural Networks (CNNs) based methods and patch-level interactions in Transformer-based methods, which are ineffective for capturing long-range dependencies. Motivated by this, we propose SEM-Net, a novel visual State Space model (SSM) vision network, modelling corrupted images at the pixel level while capturing long-range dependencies (LRDs) in state space, achieving a linear computational complexity. To address the inherent lack of spatial awareness in SSM, we introduce the Snake Mamba Block (SMB) and Spatially-Enhanced Feedforward Network. These innovations enable SEM-Net to outperform state-of-the-art inpainting methods on two distinct datasets, showing significant improvements in capturing LRDs and enhancement in spatial consistency. Additionally, SEM-Net achieves state-of-the-art performance on motion deblurring, demonstrating its generalizability. Our source code will be released in https://github.com/ChrisChen1023/SEM-Net.

==> fig/deblur.tex <==

\begin{figure*}[t]\centering
\scalebox{0.9}{
\begin{tabular}[b]{c@{ } c@{ }  c@{ } c@{ } c@{ } c@{ }	}
    \multirow{5}{*}{\includegraphics[height=.1915\textwidth,valign=t]{img/gopro/blur1.jpg}} &   
    \includegraphics[width=.143\textwidth,valign=t]{img/gopro/sharp1.jpg}&
  	\includegraphics[width=.14\textwidth,valign=t]{img/gopro/inp1.jpg}&   
      \includegraphics[width=.14\textwidth,valign=t]{img/gopro/DBGAN1.jpg}&
    \includegraphics[width=.14\textwidth,valign=t]{img/gopro/DMPHN1.jpg}&
        \includegraphics[width=.14\textwidth,valign=t]{img/gopro/Suin1.jpg}
\\
    &  \tiny~PSNR &\tiny~20.42 dB  & \tiny~23.53 dB & \tiny~24.01 dB & \tiny~21.41 dB   \\
    
    & \tiny~Reference & \tiny~Blurry    & \tiny~DBGAN \cite{zhang2020dbgan}& \tiny~DMPHN~\cite{dmphn2019}& \tiny~Suin \etal~\cite{Maitreya2020} \\

    &
    \includegraphics[width=.14\textwidth,valign=t]{img/gopro/MPRNet.jpg}&  
     \includegraphics[width=.14\textwidth,valign=t]{img/gopro/MAXIM1.jpg}&
     \includegraphics[width=.14\textwidth,valign=t]{img/gopro/Restormer1.jpg}&
    \includegraphics[width=.14\textwidth,valign=t]{img/gopro/stripformer1.jpg}&
     \includegraphics[width=.145\textwidth,valign=t]{img/gopro/sem1.jpg}\\

      & \tiny~23.15 dB 
     & \tiny~23.58 dB & \tiny 21.17 dB  & \tiny 21.92 dB & \tiny~\textbf{25.53 dB}\\
           \tiny~Blurry Image  & \tiny~MPRNet~\cite{Zamir_2021_CVPR_mprnet} & \tiny~MAXIM~\cite{tu2022maxim}   & \tiny Restormer~\cite{zamir2022restormer}& \tiny~Stripformer~\cite{tsai2022stripformer} & \tiny~\textbf{Ours}
\\
\end{tabular}
}
\caption{\small~Image motion deblurring comparisons on GoPro~\cite{gopro2017}. Our methods generates sharper and visually-faithful result.}
\label{fig:deblurring}
% \vspace{-0.5em}
\end{figure*}

==> tab/ablation.tex <==
% \usepackage{colortbl}  
% \usepackage{xcolor}
\begin{table*}[t]
\captionsetup[table]{skip=4pt}
\caption{Ablation studies of each component trained on CelebA-HQ~\cite{karras2017progressive}. }
% \captionof{table}{Ablation studies. Setup \enquote{A} replaces MPD with conventional PD, \enquote{B} removes the first FFN in \enquote{Sandwich}, \enquote{C} replaces SCAL with single channel-wise self-attention design, \enquote{D} is the full HINT.
% %\enquote{D} represents our full HINT. \enquote{A} replaces MPD with conventional PD. \enquote{B} remove the first FFN in \enquote{Sandwich}. \enquote{C} replace SCAL with single channel-wise self-attention design. MPD is Mask-aware Pixel-shuffle Down-sampling and SCAL is Squeeze-and-Channel Attention.
% }
\label{tab:ca}
	\centering
		\resizebox{\textwidth}{!}{
		{\tabulinesep=0mm
			\begin{tabu}{@{\extracolsep{3pt}} c c c c c c c c c c c | c c c c c | c c c c c@{}}
				\hline\hline
                    \multicolumn{1}{c}{\multirow{2}{*}{Net}} & 
				  \multicolumn{5}{c}{Components} & 
				\multicolumn{5}{c}{0.01\%-20\%} &
				\multicolumn{5}{c}{20\%-40\%} &
				\multicolumn{5}{c}{40\%-60\%}\T\B \\
				%\cline{2-6} \cline{7-11} \cline{12-21}
					& MB & FN~\cite{zamir2022restormer} & SEFN & SBDM & PE & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$  & LPIPS$\downarrow$\T\B\\
				\hline\hline

        % \hline
        \textbf{\textcolor{black}{(a)}} & & & & & & 33.5812 & 0.9537 & 0.5385 & 1.4877 & 0.0513 & 25.8971 & 0.8527 & 1.9786 & 4.4025 & 0.1480 & 21.6134 & 0.7308 & 4.1254 & 8.1732 & 0.2464 \\
        \textbf{\textcolor{black}{(b)}} &\checkmark &\checkmark & & & & 33.7596 & 0.9604 & 0.5274 & 1.4660 & 0.0442 & 26.0679 &0.8729 & 1.8220 & 4.3759 & 0.1261 & 21.7828 & 0.7587 & 3.9117 & 8.0742 & 0.2227\\
        \textbf{\textcolor{black}{(c)}} &\checkmark & &\checkmark & & & 34.1085 & 0.9624 & 0.5059 & 1.4147 & 0.0420 & 26.3048 & 0.8755 & 1.7299 & 4.3664 &0.1187 & 22.0510 & 0.7682 & 3.7649 & 7.9871 & 0.2132 \\ 
        \textbf{\textcolor{black}{(d)}} &\checkmark &\checkmark & &\checkmark & & 33.8899 & 0.9614 & 0.5151 & 1.4534 & 0.0415 & 26.2217 & 0.8767 & 1.7635 & 4.3674 & 0.1181 & 21.9064 & 0.7653 & 3.7679 & 8.0214 & 0.2102 \\
        % &  \textbf{\textcolor{black}{(e)}} sMamba + FN $^{\dag}$ &  & & & & & & & & & & 20.1869 & 0.7353 & 5.1323 & - & 0.1617 \\ 
        % vs self-& \textbf{\textcolor{black}{(f)}} CSA~\cite{zamir2022restormer} + FN   &  &  & & & & & & & & & - & - & - & - & -\\
        % attention& \textbf{\textcolor{black}{(g)}} SSA+ FN $^{\dag}$  &  &  & & & & & & & & & 20.1655 & 0.7265 & 5.2256 & - & 0.1702\\
        % \hline
        \textbf{\textcolor{black}{(e)}} &\checkmark & &\checkmark &\checkmark & & 34.1184 & 0.9624 & 0.5043 & 1.4010 & 0.0408 & 26.3452 & 0.8776 & 1.7155 & 4.3559 & 0.1174 & 22.0926 & 0.7692 & 3.7634  & 7.9174 & 0.2091  \\ 
        \textbf{\textcolor{black}{(f)}} &\checkmark &\checkmark & &\checkmark &\checkmark & 33.9455 & 0.9616 & 0.5128 & 1.3751 & 0.0412 & 26.4037 & 0.8790 & 1.7303 & 4.3004 & 0.1193 & 22.1776 & 0.7708 & 3.6747 & 7.9125 & 0.2095 \\ 
        \textbf{\textcolor{black}{(g)}} &\checkmark & &\checkmark &\checkmark &\checkmark & \textbf{34.1437} & \textbf{0.9627} & \textbf{0.4986} & \textbf{1.3548} & \textbf{0.0403} & \textbf{26.4728} & \textbf{0.8808} & \textbf{1.6947} & \textbf{4.2718} & \textbf{0.1145} & \textbf{22.1780} & \textbf{0.7725} & \textbf{3.6274} & \textbf{7.8915} & \textbf{0.2038}\B\\
        \hline
        \hline 
\end{tabu}
}
}
% \vspace{-0.5em}
    % \caption{Ablation studies. Setup A replaces MPD with conventional PD, B removes the first FFN in \enquote{Sandwich}, C replaces SCAL with single channel-wise self-attention design, D is the full HINT, \Chris{and E is the full HINT replacing spatial branch with the simple gated mechanism in\cite{deng2022t}.}}
% \vspace{-0.5em}
\label{tab:comp_sa}
\end{table*}

% \begin{table*}[thb]\centering
%     \caption{Ablation Study} %
%     \label{tab:ablation}
%     \resizebox{0.99  width}{!}{
%     \Large
%     \begin{tabular}{*{2}{l}||*{4}{c}||*{4}{c}||*{4}{c}}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{1}{c||}{} & \multicolumn{4}{c||}{0.01\%-20\%} & \multicolumn{4}{c||}{20\%-40\%} & \multicolumn{4}{c}{40\%-60\%} \\
%         ID & Method  & PSNRT & SSIM & L1 & LPIPS & PSNRT & SSIM & L1 & LPIPS & PSNRT & SSIM & L1 & LPIPS  \\
%         \midrule
%         A & Ours  &  {35.0436} &  {0.9671}&	 {0.4489} &	 {0.0345} &	 {27.2954} &	 {0.8924} &	 {1.5363} &	 {0.1016} &	 {22.8473} &  {0.7895} &  {3.3403} &  {0.1867} \\ %
%         B & - MPD   & 34.5955 & 0.9649 & 0.4780 & 0.0381 & 26.9292 & 0.8863 & 1.6320 & 0.1084 & 22.5618 & 0.7813 & 3.4982 & 0.1951\\
%         C & - Sandwich  & 34.7272 & 0.9658 & 0.4661 & 0.0361 & 27.0914 & 0.8893 & 1.5796 & 0.1050 & 22.7027 & 0.7853 & 3.4185 & 0.1912 \\
%         D & - SCAL & 34.7951 & 0.9659 & 0.4624 & 0.0364 & 27.1193 & 0.8895 & 1.5732 & 0.1057 & 22.7206 & .7856 & 3.4021 & 0.1925 \\        
%         \bottomrule
%     \end{tabular}
%     }


% \begin{comment}
%     \begin{table*}[ht]
% \captionsetup[table]{skip=4pt}
% \caption{Ablation studies. }
% % \captionof{table}{Ablation studies. Setup \enquote{A} replaces MPD with conventional PD, \enquote{B} removes the first FFN in \enquote{Sandwich}, \enquote{C} replaces SCAL with single channel-wise self-attention design, \enquote{D} is the full HINT.
% % %\enquote{D} represents our full HINT. \enquote{A} replaces MPD with conventional PD. \enquote{B} remove the first FFN in \enquote{Sandwich}. \enquote{C} replace SCAL with single channel-wise self-attention design. MPD is Mask-aware Pixel-shuffle Down-sampling and SCAL is Squeeze-and-Channel Attention.
% % }
% % \label{tab:ablation}
% 	\centering
% 		\resizebox{\columnwidth}{!}{
% 		{\tabulinesep=0mm
% 			\begin{tabu}{@{\extracolsep{3pt}} c | c c c c c c | c c c c c | c c c c c@{}}
% 				\hline\hline
% 				\multicolumn{1}{c}{\multirow{2}{*}{Setup}} & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
% 				\multicolumn{5}{c}{0.01\%-20\%} &
% 				\multicolumn{5}{c}{20\%-40\%} &
% 				\multicolumn{5}{c}{40\%-60\%}\T\B \\
% 				\cline{3-7} \cline{8-12} \cline{13-17}
% 						&& PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$  & LPIPS$\downarrow$\T\B\\
% 				\hline\hline

%         % \hline
%         Baseline & \textbf{\textcolor{black}{(a)}}UNet-MB & 33.5812 & 0.9537 & 0.5385 & 1.4877 & 0.0513 & 25.8971 & 0.8527 & 1.9786 & 4.4025 & 0.1480 & 21.6134 & 0.7308 & 4.1254 & 8.1732 & 0.2464 \\
%         \hline
%         Snack & \textbf{\textcolor{black}{(b)}} MB+FN   & 33.7596 & 0.9604 & 0.5274 & 1.4660 & 0.0442 & 26.0679 &0.8729 & 1.8220 & 4.3759 & 0.1261 & 21.7828 & 0.7587 & 3.9117 & 8.0742 & 0.2227\\
%         Mamba & \textbf{\textcolor{black}{(c)}} MB+SBDM+FN &  33.8899 & 0.9614 & 0.5151 & 1.4534 & 0.0415 & 26.2217 & 0.8767 & 1.7635 & 4.3674 & 0.1181 & 21.9064 & 0.7653 & 3.7679 & 8.0214 & 0.2102 \\
%         Block & \textbf{\textcolor{black}{(d)}} MB+SBDM+PE+FN & 33.9455 & 0.9616 & 0.5128 & 1.3751 & 0.0431 & 26.4037 & 0.8790 & 1.7303 & 4.3004 & 0.1193 & 22.1776 & 0.7708 & 3.6747 & 7.9125 & 0.2095 \\ 
%         % &  \textbf{\textcolor{black}{(e)}} sMamba + FN $^{\dag}$ &  & & & & & & & & & & 20.1869 & 0.7353 & 5.1323 & - & 0.1617 \\ 
%         \hline
%         % vs self-& \textbf{\textcolor{black}{(f)}} CSA~\cite{zamir2022restormer} + FN   &  &  & & & & & & & & & - & - & - & - & -\\
%         % attention& \textbf{\textcolor{black}{(g)}} SSA+ FN $^{\dag}$  &  &  & & & & & & & & & 20.1655 & 0.7265 & 5.2256 & - & 0.1702\\
%         % \hline
%         SE& \textbf{\textcolor{black}{(e)}} MB+SEFN & 34.1085 & 0.9624 & 0.5059 & 1.4147 & 0.04201 & 26.3048 & 0.8755 & 1.7299 & 4.3664 &0.1187 & 22.0510 & 0.7682 & 3.7649 & 7.9871 & 0.2132 \\ 
%         FN& \textbf{\textcolor{black}{(f)}} MB+SBDM+SEFN & 34.1184 & 0.9624 & 0.5043 & 1.4010 & 0.0408 & 26.3452 & 0.8776 & 1.7155 & 4.3559 & 0.1174 & 22.0926 & 0.7692 & 3.7634  & 7.9174 & 0.2091  \\ 
%         \hline
%         Ours & \textbf{\textcolor{black}{(g)}} MB+SBDM+PE+SEFN  & \textbf{34.1437} & \textbf{0.9627} & \textbf{0.4986} & \textbf{1.3548} & \textbf{0.0403} & \textbf{26.4728} & \textbf{0.8808} & \textbf{1.6947} & \textbf{4.2718} & \textbf{0.1145} & \textbf{22.1780} & \textbf{0.7725} & \textbf{3.6274} & \textbf{7.8915} & \textbf{0.2038}\B\\
%         \hline
%         \hline 
% \end{tabu}
% }
% }
% % \vspace{-0.5em}
%     % \caption{Ablation studies. Setup A replaces MPD with conventional PD, B removes the first FFN in \enquote{Sandwich}, C replaces SCAL with single channel-wise self-attention design, D is the full HINT, \Chris{and E is the full HINT replacing spatial branch with the simple gated mechanism in\cite{deng2022t}.}}
% \vspace{-0.5em}
% \label{tab:ablation}
% \end{table*}
% \end{comment}

% %%hz
% \begin{comment}
%     \begin{table*}[ht]
% \captionsetup[table]{skip=4pt}
% \caption{Ablation studies. }
% % \captionof{table}{Ablation studies. Setup \enquote{A} replaces MPD with conventional PD, \enquote{B} removes the first FFN in \enquote{Sandwich}, \enquote{C} replaces SCAL with single channel-wise self-attention design, \enquote{D} is the full HINT.
% % %\enquote{D} represents our full HINT. \enquote{A} replaces MPD with conventional PD. \enquote{B} remove the first FFN in \enquote{Sandwich}. \enquote{C} replace SCAL with single channel-wise self-attention design. MPD is Mask-aware Pixel-shuffle Down-sampling and SCAL is Squeeze-and-Channel Attention.
% % }
% % \label{tab:ablation}
% 	\centering
% 		\resizebox{\columnwidth}{!}{
% 		{\tabulinesep=0mm
% 			\begin{tabu}{@{\extracolsep{3pt}}  l c c c c c | c c c c c | c c c c c@{}}
% 				\hline\hline
% 				  \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
% 				\multicolumn{5}{c}{0.01\%-20\%} &
% 				\multicolumn{5}{c}{20\%-40\%} &
% 				\multicolumn{5}{c}{40\%-60\%}\T\B \\
% 				\cline{2-6} \cline{7-11} \cline{12-16}
% 						& PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$  & LPIPS$\downarrow$\T\B\\
% 				\hline\hline

%         % \hline
%         \textbf{\textcolor{black}{(a)}} UNet-MB (Baseline) & 33.5812 & 0.9537 & 0.5385 & 1.4877 & 0.0513 & 25.8971 & 0.8527 & 1.9786 & 4.4025 & 0.1480 & 21.6134 & 0.7308 & 4.1254 & 8.1732 & 0.2464 \\
%         \textbf{\textcolor{black}{(b)}} MB+FN~\cite{zamir2022restormer}   & 33.7596 & 0.9604 & 0.5274 & 1.4660 & 0.0442 & 26.0679 &0.8729 & 1.8220 & 4.3759 & 0.1261 & 21.7828 & 0.7587 & 3.9117 & 8.0742 & 0.2227\\
%         \textbf{\textcolor{black}{(c)}} MB+SEFN & 34.1085 & 0.9624 & 0.5059 & 1.4147 & 0.04201 & 26.3048 & 0.8755 & 1.7299 & 4.3664 &0.1187 & 22.0510 & 0.7682 & 3.7649 & 7.9871 & 0.2132 \\ 
%         \textbf{\textcolor{black}{(d)}} MB+FN~\cite{zamir2022restormer}+SBDM &  33.8899 & 0.9614 & 0.5151 & 1.4534 & 0.0415 & 26.2217 & 0.8767 & 1.7635 & 4.3674 & 0.1181 & 21.9064 & 0.7653 & 3.7679 & 8.0214 & 0.2102 \\
%         % &  \textbf{\textcolor{black}{(e)}} sMamba + FN $^{\dag}$ &  & & & & & & & & & & 20.1869 & 0.7353 & 5.1323 & - & 0.1617 \\ 
%         % vs self-& \textbf{\textcolor{black}{(f)}} CSA~\cite{zamir2022restormer} + FN   &  &  & & & & & & & & & - & - & - & - & -\\
%         % attention& \textbf{\textcolor{black}{(g)}} SSA+ FN $^{\dag}$  &  &  & & & & & & & & & 20.1655 & 0.7265 & 5.2256 & - & 0.1702\\
%         % \hline
%         \textbf{\textcolor{black}{(e)}} MB+SEFN+SBDM & 34.1184 & 0.9624 & 0.5043 & 1.4010 & 0.0408 & 26.3452 & 0.8776 & 1.7155 & 4.3559 & 0.1174 & 22.0926 & 0.7692 & 3.7634  & 7.9174 & 0.2091  \\ 
%         \textbf{\textcolor{black}{(f)}} MB+FN~\cite{zamir2022restormer}+SBDM+PE & 33.9455 & 0.9616 & 0.5128 & 1.3751 & 0.0412 & 26.4037 & 0.8790 & 1.7303 & 4.3004 & 0.1193 & 22.1776 & 0.7708 & 3.6747 & 7.9125 & 0.2095 \\ 
%         \hline
%         \textbf{\textcolor{black}{(g)}} MB+SEFN+SBDM+PE (Ours) & \textbf{34.1437} & \textbf{0.9627} & \textbf{0.4986} & \textbf{1.3548} & \textbf{0.0403} & \textbf{26.4728} & \textbf{0.8808} & \textbf{1.6947} & \textbf{4.2718} & \textbf{0.1145} & \textbf{22.1780} & \textbf{0.7725} & \textbf{3.6274} & \textbf{7.8915} & \textbf{0.2038}\B\\
%         \hline
%         \hline 
% \end{tabu}
% }
% }
% % \vspace{-0.5em}
%     % \caption{Ablation studies. Setup A replaces MPD with conventional PD, B removes the first FFN in \enquote{Sandwich}, C replaces SCAL with single channel-wise self-attention design, D is the full HINT, \Chris{and E is the full HINT replacing spatial branch with the simple gated mechanism in\cite{deng2022t}.}}
% \vspace{-0.5em}
% \label{tab:ablation}
% \end{table*}
% \end{comment}

==> tab/deblur_wacv.tex <==
\begin{table}[htbp]
        \centering
        \caption{Number of parameters and inference time, based on the inpainting evaluation conducted on $256\times256$ images.\\}
        \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{ccc}
        \hline\hline
        % \hline
        Model & Param $\times 10^6$ & Infer. Time/per img\T\B\\
        \hline
        % DeepFill v1 \cite{yu2018generative} & 3 & 7 $ms$\T \\
        % DeepFill v2 \cite{yu2019free} & 4 & 10 $ms$ \\
        Wavefill \cite{yu2021wavefill} & 49 & 70 $ms$ \T\\
        CTSDG \cite{guo2021image} & 52 & 20 $ms$\\
        WNet \cite{zhang2022w} & 46 & 35 $ms$\\
        MISF \cite{li2022misf} & 26 & 10 $ms$ \\
        MAT \cite{li2022mat} & 62 & 70 $ms$ \\
        CMT \cite{ko2023continuously} & 143 & 60 $ms$\\
        LAMA \cite{suvorov2022resolution} & 51 & 25 $ms$ \\
        \small{Stable Diffusion~\cite{Rombach_2022_CVPR}} & 860 & 880 $ms$\\
        LDM~\cite{Rombach_2022_CVPR} & 387 & ~6000 $ms$\\
        Repaint~\cite{Lugmayr_2022_CVPR} & 552 & ~250000 $ms$\B\\
        \hline
        {Ours} & {163} & {200} $ms$\T\B\\
        \hline\hline
        % \hline
        \end{tabular}
        \end{adjustbox}
        \label{tab:inf_time}
\end{table}

==> tab/diff.tex <==
\begin{table}[t]\centering
\captionsetup[table]{skip=4pt}
\caption{Comparison with diffusion models.}
\scriptsize
\label{tab:diffusion}
    \tabulinesep=0mm
    \begin{tabular}{*{6}{c}}
    \hline\hline
    Plces2 &  PSNR$\uparrow$ & SSIM$\uparrow$ &  L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$\T\B\\
    \hline
    LDM~\cite{Rombach_2022_CVPR} & 19.6476 & 0.7052 & 4.6895 & 27.3619 & 0.2675\T\\
    Stable Diffusion$^*$ & 19.4812 & 0.7185 & 4.5729 & 27.8830 & 0.2416\\
    Ours & \textbf{20.8265} & \textbf{0.7279} & \textbf{4.3614} & \textbf{25.7049} & \textbf{0.2148} \\
    \hline
    \hline
    CelebA-HQ &  PSNR$\uparrow$ & SSIM$\uparrow$ &  L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$\T\B\\
    \hline
    RePaint~\cite{Lugmayr_2022_CVPR} & 21.8321 & 0.7791 & 3.9427 & 8.9637 & 0.1943 \T\\
    Ours &\textbf{24.4805} & \textbf{0.8240} & \textbf{2.6389} & \textbf{5.5972} &\textbf{0.1368}\\
    \hline\hline
    \multicolumn{6}{l}{\small $^*$: The officially released Stable Diffusion inpainting model} \T\\
    \multicolumn{6}{l}{\small pretrained on high-quality LAION-Aesthetics V2 5+ dataset.} \\
    \end{tabular}
    % \vspace{-4.5em}
\end{table}

==> tab/time_deblurr.tex <==
\begin{table}[htbp]
    \centering
    % \captionsetup[table]{skip=4pt}
        \caption{Number of parameters and inference time, based on the inpainting evaluation conducted on $256\times256$ images.}
        \scalebox{0.8}{
        % {width=0.9 * \linewidth}
        \begin{tabular}{ccc}
        \hline\hline
        % \hline
        Model & Param $\times 10^6$ & Infer. Time/per img\T\B\\
        \hline
        % DeepFill v1 \cite{yu2018generative} & 3 & 7 $ms$\T \\
        % DeepFill v2 \cite{yu2019free} & 4 & 10 $ms$ \\
        Wavefill \cite{yu2021wavefill} & 49 & 70 $ms$ \T\\
        CTSDG \cite{guo2021image} & 52 & 20 $ms$\\
        % WNet \cite{zhang2022w} & 46 & 35 $ms$\\
        MISF \cite{li2022misf} & 26 & 10 $ms$ \\
        MAT \cite{li2022mat} & 62 & 70 $ms$ \\
        CMT \cite{ko2023continuously} & 143 & 60 $ms$\\
        LAMA \cite{suvorov2022resolution} & 51 & 25 $ms$ \\
        \small{Stable Diffusion~\cite{Rombach_2022_CVPR}} & 860 & 880 $ms$\\
        LDM~\cite{Rombach_2022_CVPR} & 387 & 6000 $ms$\\
        Repaint~\cite{Lugmayr_2022_CVPR} & 552 & ~250000 $ms$\B\\
        \hline
        {Ours} & {163} & {240} $ms$\T\B\\
        \hline\hline
        % \hline
        \end{tabular}}
        % \end{adjustbox}
        \label{tab:inf_time}
\end{table}

==> tab/vcSA.tex <==
% \usepackage{colortbl}  
% \usepackage{xcolor}
\begin{table*}[t]
\captionsetup[table]{skip=4pt}
\caption{Comparison between our proposed SMB with transformer-based methods.}
% \captionof{table}{Ablation studies. Setup \enquote{A} replaces MPD with conventional PD, \enquote{B} removes the first FFN in \enquote{Sandwich}, \enquote{C} replaces SCAL with single channel-wise self-attention design, \enquote{D} is the full HINT.
% %\enquote{D} represents our full HINT. \enquote{A} replaces MPD with conventional PD. \enquote{B} remove the first FFN in \enquote{Sandwich}. \enquote{C} replace SCAL with single channel-wise self-attention design. MPD is Mask-aware Pixel-shuffle Down-sampling and SCAL is Squeeze-and-Channel Attention.
% }
% \label{tab:ablation}
	\centering
		\resizebox{\textwidth}{!}{
		{\tabulinesep=0mm
			\begin{tabu}{@{\extracolsep{3pt}} c  c c c c c c | c c c c c | c c c c c@{}}
				\hline\hline
				\multicolumn{1}{c}{\multirow{1}{*}{Input}} & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
				\multicolumn{5}{c}{0.01\%-20\%} &
				\multicolumn{5}{c}{20\%-40\%} &
				\multicolumn{5}{c}{40\%-60\%}\T\B \\
				\cline{3-7} \cline{8-12} \cline{13-17}
					Resolution& & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$  & LPIPS$\downarrow$\T\B\\
				\hline\hline
        \multicolumn{1}{c}{\multirow{3}{*}{256*256}}& CSA~\cite{zamir2022restormer}   & 33.5878 & 0.9595 & 0.5451 & 2.7514 & 0.0462 & 25.9348 & 0.8712 & 1.8644 & 5.1404 & 0.1300 & 21.5362 & 0.7543 & 4.0471 & 8.1652 & 0.2326\\
        & SSA~\cite{dosovitskiy2020image} & \multicolumn{5}{c}{\multirow{1}{*}{Out of memory}}& \multicolumn{5}{c}{\multirow{1}{*}{Out of memory}}&  \multicolumn{5}{c}{\multirow{1}{*}{Out of memory}}\\
         & SMB & \textbf{33.9455} & \textbf{0.9616} & \textbf{0.512}8 & \textbf{1.3751} & \textbf{0.0431} & \textbf{26.4037} & \textbf{0.8790} & \textbf{1.7303} & \textbf{4.3004} & \textbf{0.1193} & \textbf{22.1776} & \textbf{0.7708} & \textbf{3.6747} & \textbf{7.9125} & \textbf{0.2095} \\  
        \hline
        \hline
        \multicolumn{1}{c}{\multirow{2}{*}{64*64}}& SSA~\cite{dosovitskiy2020image} & 32.0110 & 0.9308 & 0.7354 & 0.8345 & 0.0375 & 24.5320 & 0.7121 &3.3047 & 2.8991 & 0.1035 & 20.1655 & 0.7265 & 5.2256 & 5.5547 & 0.1702\\
        & SMB & \textbf{32.0218} & \textbf{0.9437} & \textbf{0.7120} & \textbf{0.8152} & \textbf{0.0351} & \textbf{24.6112} & \textbf{0.7214} & \textbf{3.1575} & \textbf{2.7503} & \textbf{0.1022} & \textbf{20.1716} & \textbf{0.7352} & \textbf{5.1332} & \textbf{5.3158} & \textbf{0.1617}\B\\
        \hline
        \hline 
\end{tabu}
}
}
% \vspace{-0.5em}
    % \caption{Ablation studies. Setup A replaces MPD with conventional PD, B removes the first FFN in \enquote{Sandwich}, C replaces SCAL with single channel-wise self-attention design, D is the full HINT, \Chris{and E is the full HINT replacing spatial branch with the simple gated mechanism in\cite{deng2022t}.}}
% \vspace{-0.5em}
\label{tab:ablation}
\end{table*}

% \begin{table*}[thb]\centering
%     \caption{Ablation Study} %
%     \label{tab:ablation}
%     \resizebox{0.99  width}{!}{
%     \Large
%     \begin{tabular}{*{2}{l}||*{4}{c}||*{4}{c}||*{4}{c}}
%         \toprule
%         \multicolumn{1}{c}{} & \multicolumn{1}{c||}{} & \multicolumn{4}{c||}{0.01\%-20\%} & \multicolumn{4}{c||}{20\%-40\%} & \multicolumn{4}{c}{40\%-60\%} \\
%         ID & Method  & PSNRT & SSIM & L1 & LPIPS & PSNRT & SSIM & L1 & LPIPS & PSNRT & SSIM & L1 & LPIPS  \\
%         \midrule
%         A & Ours  &  {35.0436} &  {0.9671}&	 {0.4489} &	 {0.0345} &	 {27.2954} &	 {0.8924} &	 {1.5363} &	 {0.1016} &	 {22.8473} &  {0.7895} &  {3.3403} &  {0.1867} \\ %
%         B & - MPD   & 34.5955 & 0.9649 & 0.4780 & 0.0381 & 26.9292 & 0.8863 & 1.6320 & 0.1084 & 22.5618 & 0.7813 & 3.4982 & 0.1951\\
%         C & - Sandwich  & 34.7272 & 0.9658 & 0.4661 & 0.0361 & 27.0914 & 0.8893 & 1.5796 & 0.1050 & 22.7027 & 0.7853 & 3.4185 & 0.1912 \\
%         D & - SCAL & 34.7951 & 0.9659 & 0.4624 & 0.0364 & 27.1193 & 0.8895 & 1.5732 & 0.1057 & 22.7206 & .7856 & 3.4021 & 0.1925 \\        
%         \bottomrule
%     \end{tabular}
%     }


% \begin{comment}
%     \begin{table*}[ht]
% \captionsetup[table]{skip=4pt}
% \caption{Comparison with self-attention}
% % \captionof{table}{Ablation studies. Setup \enquote{A} replaces MPD with conventional PD, \enquote{B} removes the first FFN in \enquote{Sandwich}, \enquote{C} replaces SCAL with single channel-wise self-attention design, \enquote{D} is the full HINT.
% % %\enquote{D} represents our full HINT. \enquote{A} replaces MPD with conventional PD. \enquote{B} remove the first FFN in \enquote{Sandwich}. \enquote{C} replace SCAL with single channel-wise self-attention design. MPD is Mask-aware Pixel-shuffle Down-sampling and SCAL is Squeeze-and-Channel Attention.
% % }
% % \label{tab:ablation}
% 	\centering
% 		\resizebox{\columnwidth}{!}{
% 		{\tabulinesep=0mm
% 			\begin{tabu}{@{\extracolsep{3pt}} c | c c c c c c | c c c c c | c c c c c@{}}
% 				\hline\hline
% 				\multicolumn{1}{c}{\multirow{2}{*}{Setup}} & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & 
% 				\multicolumn{5}{c}{0.01\%-20\%} &
% 				\multicolumn{5}{c}{20\%-40\%} &
% 				\multicolumn{5}{c}{40\%-60\%}\T\B \\
% 				\cline{3-7} \cline{8-12} \cline{13-17}
% 						&& PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & L1$\downarrow$ & FID$\downarrow$  & LPIPS$\downarrow$\T\B\\
% 				\hline\hline
%         vs self-& CSA~\cite{zamir2022restormer} + FN   & 33.5878 & 0.9595 & 0.5451 & 2.7514 & 0.0462 & 25.9348 & 0.8712 & 1.8644 & 5.1404 & 0.1300 & 21.5362 & 0.7543 & 4.0471 & 8.1652 & 0.2326\\
%         attention & SSA+ FN $^{\dag}$  & 32.0110 & 0.9308 & 0.7354 & 0.8345 & 0.0375 & 24.5320 & 0.7121 &3.3047 & 2.8991 & 24.5320 & 20.1655 & 0.7265 & 5.2256 & 5.5547 & 0.1702\\
%         \hline
%         \hline
%         Ours & SMB + FN & 33.9455 & 0.9616 & 0.5128 & 1.3751 & 0.0431 & 26.4037 & 0.8790 & 1.7303 & 4.3004 & 0.1193 & 22.1776 & 0.7708 & 3.6747 & 7.9125 & 0.2095 \\
%         Ours$^{\dag}$ & SMB + FN $^{\dag}$  & 32.0218 & 0.9437 & 0.7120 & 0.8152 & 0.0351 & 24.6112 & 0.7214 & 3.1575 & 2.7503 & 0.1193 & 20.1716 & 0.7352 & 5.1332 & 5.3158 & 0.1617 \B\\
%         \hline
%         \hline 
% \end{tabu}
% }
% }
% % \vspace{-0.5em}
%     % \caption{Ablation studies. Setup A replaces MPD with conventional PD, B removes the first FFN in \enquote{Sandwich}, C replaces SCAL with single channel-wise self-attention design, D is the full HINT, \Chris{and E is the full HINT replacing spatial branch with the simple gated mechanism in\cite{deng2022t}.}}
% \vspace{-0.5em}
% \label{tab:ablation}
% \end{table*}
% \end{comment}
